Pre-training with Synthetic Data Helps Offline Reinforcement Learning

Recently, it has been shown that for offline deep reinforcement learning (DRL), pre-training Decision Transformer with a large language corpus can improve downstream performance (Reid et al., 2022). A natural question to ask is whether this performance gain can only be achieved with language pre-training, or can be achieved with simpler pre-training schemes which do not involve language. In this paper, we first show that language is not essential for improved performance, and indeed pre-training with synthetic IID data for a small number of updates can match the performance gains from pre-training with a large language corpus; moreover, pre-training with data generated by a one-step Markov chain can further improve the performance. Inspired by these experimental results, we then consider pre-training Conservative Q-Learning (CQL), a popular offline DRL algorithm, which is Q-learning-based and typically employs a Multi-Layer Perceptron (MLP) backbone. Surprisingly, pre-training with simple synthetic data for a small number of updates can also improve CQL, providing consistent performance improvement on D4RL Gym locomotion datasets. The results of this paper not only illustrate the importance of pre-training for offline DRL but also show that the pre-training data can be synthetic and generated with remarkably simple mechanisms.

==> cql_new_figures/antmaze.tex <==
\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{cql_new_figures/all_figures/agg-cql_antmaze_subopt_TestEpNormRet.png}
\caption{Performance curve of each setting averaged over 12 datasets.}
\label{fig:cql-performance-agg-curves}
\end{figure}

\begin{figure}[htb]
\captionsetup[subfigure]{justification=centering}
\centering
\begin{subfigure}[t]{.32\linewidth}
\centering
\includegraphics[width=\linewidth]{cql_new_figures/all_figures/ind-cql_antmaze_subopt_TestEpNormRet_antmaze-umaze_play.png}
\caption{Antmaze-umaze-play}
\end{subfigure}
\begin{subfigure}[t]{.32\linewidth}
\centering
\includegraphics[width=\linewidth]{cql_new_figures/all_figures/ind-cql_antmaze_subopt_TestEpNormRet_antmaze-medium_play.png}
\caption{Antmaze-medium-play}
\end{subfigure}
\begin{subfigure}[t]{.32\linewidth}
\centering
\includegraphics[width=\linewidth]{cql_new_figures/all_figures/ind-cql_antmaze_subopt_TestEpNormRet_antmaze-large_play.png}
\caption{Antmaze-large-play}
\end{subfigure}\\
\begin{subfigure}[t]{.32\linewidth}
\centering
\includegraphics[width=\linewidth]{cql_new_figures/all_figures/ind-cql_antmaze_subopt_TestEpNormRet_antmaze-umaze_diverse.png}
\caption{Antmaze-umaze-diverse}
\end{subfigure}
\begin{subfigure}[t]{.32\linewidth}
\centering
\includegraphics[width=\linewidth]{cql_new_figures/all_figures/ind-cql_antmaze_subopt_TestEpNormRet_antmaze-medium_diverse.png}
\caption{Antmaze-medium-diverse}
\end{subfigure}
\begin{subfigure}[t]{.32\linewidth}
\centering
\includegraphics[width=\linewidth]{cql_new_figures/all_figures/ind-cql_antmaze_subopt_TestEpNormRet_antmaze-large_diverse.png}
\caption{Antmaze-large-diverse}
\end{subfigure}\\
\caption{Learning curves for CQL, CQL with same task RL data pretraining, and CQL with MDP pretraining.}
\label{fig:cql-performance-curves}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=\linewidth]{cql_new_figures/all_figures/agg-cql_antmaze_tuned_a3_TestEpNormRet.png}
\caption{Performance curve of each setting averaged over 12 datasets.}
\label{fig:cql-performance-agg-curves}
\end{figure}

\begin{figure}[htb]
\captionsetup[subfigure]{justification=centering}
\centering
\begin{subfigure}[t]{.32\linewidth}
\centering
\includegraphics[width=\linewidth]{cql_new_figures/all_figures/ind-cql_antmaze_tuned_a3_TestEpNormRet_antmaze-umaze_play.png}
\caption{Antmaze-umaze-play}
\end{subfigure}
\begin{subfigure}[t]{.32\linewidth}
\centering
\includegraphics[width=\linewidth]{cql_new_figures/all_figures/ind-cql_antmaze_tuned_a3_TestEpNormRet_antmaze-medium_play.png}
\caption{Antmaze-medium-play}
\end{subfigure}
\begin{subfigure}[t]{.32\linewidth}
\centering
\includegraphics[width=\linewidth]{cql_new_figures/all_figures/ind-cql_antmaze_tuned_a3_TestEpNormRet_antmaze-large_play.png}
\caption{Antmaze-large-play}
\end{subfigure}\\
\begin{subfigure}[t]{.32\linewidth}
\centering
\includegraphics[width=\linewidth]{cql_new_figures/all_figures/ind-cql_antmaze_tuned_a3_TestEpNormRet_antmaze-umaze_diverse.png}
\caption{Antmaze-umaze-diverse}
\end{subfigure}
\begin{subfigure}[t]{.32\linewidth}
\centering
\includegraphics[width=\linewidth]{cql_new_figures/all_figures/ind-cql_antmaze_tuned_a3_TestEpNormRet_antmaze-medium_diverse.png}
\caption{Antmaze-medium-diverse}
\end{subfigure}
\begin{subfigure}[t]{.32\linewidth}
\centering
\includegraphics[width=\linewidth]{cql_new_figures/all_figures/ind-cql_antmaze_tuned_a3_TestEpNormRet_antmaze-large_diverse.png}
\caption{Antmaze-large-diverse}
\end{subfigure}\\
\caption{Learning curves for CQL, CQL with same task RL data pretraining, and CQL with MDP pretraining.}
\label{fig:cql-performance-curves}
\end{figure}

==> extra.tex <==


\begin{comment}

\begin{figure}[htb]
\centering
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-offset-new-new_current_itr_train_loss_mean_hopper_medium.png}
\caption{Hopper-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-offset-new-new_current_itr_train_loss_mean_hopper_medium-replay.png}
\caption{Hopper-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-offset-new-new_current_itr_train_loss_mean_hopper_medium-expert.png}
\caption{Hopper-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-offset-new-new_current_itr_train_loss_mean_walker2d_medium.png}
\caption{Walker-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-offset-new-new_current_itr_train_loss_mean_walker2d_medium-replay.png}
\caption{Walker-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-offset-new-new_current_itr_train_loss_mean_walker2d_medium-expert.png}
\caption{Walker-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-offset-new-new_current_itr_train_loss_mean_halfcheetah_medium.png}
\caption{HalfCheetah-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-offset-new-new_current_itr_train_loss_mean_halfcheetah_medium-replay.png}
\caption{HalfCheetah-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-offset-new-new_current_itr_train_loss_mean_halfcheetah_medium-expert.png}
\caption{HalfCheetah-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-offset-new-new_current_itr_train_loss_mean_ant_medium.png}
\caption{Ant-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-offset-new-new_current_itr_train_loss_mean_ant_medium-replay.png}
\caption{Ant-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-offset-new-new_current_itr_train_loss_mean_ant_medium-expert.png}
\caption{Ant-medium-expert}
\end{subfigure}
\caption{Loss curves of individual datasets for DT, DT+Wiki, DT+Synthetic. The DT baseline is fine-tuned for 180K updates. To account for the pre-training updates, we offset the curves for DT+Synthetic to the right by 20K updates and fine-tune for 160K updates, and we offset the curve for DT+Wiki to the right by 80K updates and fine-tune for 100K updates.}
\label{fig:dt-loss-curves-offset-new}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}[htb]
\centering
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-states_TestEpNormRet_hopper_medium.png}
\caption{Hopper-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-states_TestEpNormRet_hopper_medium-replay.png}
\caption{Hopper-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-states_TestEpNormRet_hopper_medium-expert.png}
\caption{Hopper-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-states_TestEpNormRet_walker2d_medium.png}
\caption{Walker-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-states_TestEpNormRet_walker2d_medium-replay.png}
\caption{Walker-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-states_TestEpNormRet_walker2d_medium-expert.png}
\caption{Walker-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-states_TestEpNormRet_halfcheetah_medium.png}
\caption{HalfCheetah-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-states_TestEpNormRet_halfcheetah_medium-replay.png}
\caption{HalfCheetah-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-states_TestEpNormRet_halfcheetah_medium-expert.png}
\caption{HalfCheetah-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-states_TestEpNormRet_ant_medium.png}
\caption{Ant-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-states_TestEpNormRet_ant_medium-replay.png}
\caption{Ant-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-states_TestEpNormRet_ant_medium-expert.png}
\caption{Ant-medium-expert}
\end{subfigure}

\caption{Ablations for impact of state, MC steps and temperature hyper-parameters on performance for different amounts of  fine-tuning updates for individual datasets.}
\label{fig:dt-learning-curves-agg-ft-states}
\end{figure}

\begin{figure}[htb]
\centering
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-step_TestEpNormRet_hopper_medium.png}
\caption{Hopper-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-step_TestEpNormRet_hopper_medium-replay.png}
\caption{Hopper-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-step_TestEpNormRet_hopper_medium-expert.png}
\caption{Hopper-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-step_TestEpNormRet_walker2d_medium.png}
\caption{Walker-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-step_TestEpNormRet_walker2d_medium-replay.png}
\caption{Walker-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-step_TestEpNormRet_walker2d_medium-expert.png}
\caption{Walker-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-step_TestEpNormRet_halfcheetah_medium.png}
\caption{HalfCheetah-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-step_TestEpNormRet_halfcheetah_medium-replay.png}
\caption{HalfCheetah-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-step_TestEpNormRet_halfcheetah_medium-expert.png}
\caption{HalfCheetah-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-step_TestEpNormRet_ant_medium.png}
\caption{Ant-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-step_TestEpNormRet_ant_medium-replay.png}
\caption{Ant-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-step_TestEpNormRet_ant_medium-expert.png}
\caption{Ant-medium-expert}
\end{subfigure}

\caption{Ablations of state, MC step and temperature against finetuning updates for individual datasets.}
\label{fig:dt-learning-curves-agg-ft-step}
\end{figure}



\begin{figure}[htb]
\centering
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-temp_TestEpNormRet_hopper_medium.png}
\caption{Hopper-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-temp_TestEpNormRet_hopper_medium-replay.png}
\caption{Hopper-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-temp_TestEpNormRet_hopper_medium-expert.png}
\caption{Hopper-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-temp_TestEpNormRet_walker2d_medium.png}
\caption{Walker-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-temp_TestEpNormRet_walker2d_medium-replay.png}
\caption{Walker-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-temp_TestEpNormRet_walker2d_medium-expert.png}
\caption{Walker-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-temp_TestEpNormRet_halfcheetah_medium.png}
\caption{HalfCheetah-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-temp_TestEpNormRet_halfcheetah_medium-replay.png}
\caption{HalfCheetah-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-temp_TestEpNormRet_halfcheetah_medium-expert.png}
\caption{HalfCheetah-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-temp_TestEpNormRet_ant_medium.png}
\caption{Ant-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-temp_TestEpNormRet_ant_medium-replay.png}
\caption{Ant-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftsteps-temp_TestEpNormRet_ant_medium-expert.png}
\caption{Ant-medium-expert}
\end{subfigure}

\caption{Ablations of state, MC step and temperature against finetuning updates for individual datasets.}
\label{fig:dt-learning-curves-agg-ft-temp}
\end{figure}





\begin{figure}[htb]
\centering
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-states_TestEpNormRet_hopper_medium.png}
\caption{Hopper-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-states_TestEpNormRet_hopper_medium-replay.png}
\caption{Hopper-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-states_TestEpNormRet_hopper_medium-expert.png}
\caption{Hopper-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-states_TestEpNormRet_walker2d_medium.png}
\caption{Walker-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-states_TestEpNormRet_walker2d_medium-replay.png}
\caption{Walker-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-states_TestEpNormRet_walker2d_medium-expert.png}
\caption{Walker-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-states_TestEpNormRet_halfcheetah_medium.png}
\caption{HalfCheetah-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-states_TestEpNormRet_halfcheetah_medium-replay.png}
\caption{HalfCheetah-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-states_TestEpNormRet_halfcheetah_medium-expert.png}
\caption{HalfCheetah-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-states_TestEpNormRet_ant_medium.png}
\caption{Ant-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-states_TestEpNormRet_ant_medium-replay.png}
\caption{Ant-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-states_TestEpNormRet_ant_medium-expert.png}
\caption{Ant-medium-expert}
\end{subfigure}

\caption{Ablations of state, MC step and temperature against finetuning updates for individual datasets.}
\label{fig:dt-learning-curves-agg-ftratio-states}
\end{figure}




\begin{figure}[htb]
\centering
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-step_TestEpNormRet_hopper_medium.png}
\caption{Hopper-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-step_TestEpNormRet_hopper_medium-replay.png}
\caption{Hopper-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-step_TestEpNormRet_hopper_medium-expert.png}
\caption{Hopper-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-step_TestEpNormRet_walker2d_medium.png}
\caption{Walker-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-step_TestEpNormRet_walker2d_medium-replay.png}
\caption{Walker-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-step_TestEpNormRet_walker2d_medium-expert.png}
\caption{Walker-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-step_TestEpNormRet_halfcheetah_medium.png}
\caption{HalfCheetah-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-step_TestEpNormRet_halfcheetah_medium-replay.png}
\caption{HalfCheetah-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-step_TestEpNormRet_halfcheetah_medium-expert.png}
\caption{HalfCheetah-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-step_TestEpNormRet_ant_medium.png}
\caption{Ant-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-step_TestEpNormRet_ant_medium-replay.png}
\caption{Ant-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-step_TestEpNormRet_ant_medium-expert.png}
\caption{Ant-medium-expert}
\end{subfigure}

\caption{Ablations of state, MC step and temperature against finetuning updates for individual datasets.}
\label{fig:dt-learning-curves-agg-ftratio-step}
\end{figure}




\begin{figure}[htb]
\centering
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-temp_TestEpNormRet_hopper_medium.png}
\caption{Hopper-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-temp_TestEpNormRet_hopper_medium-replay.png}
\caption{Hopper-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-temp_TestEpNormRet_hopper_medium-expert.png}
\caption{Hopper-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-temp_TestEpNormRet_walker2d_medium.png}
\caption{Walker-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-temp_TestEpNormRet_walker2d_medium-replay.png}
\caption{Walker-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-temp_TestEpNormRet_walker2d_medium-expert.png}
\caption{Walker-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-temp_TestEpNormRet_halfcheetah_medium.png}
\caption{HalfCheetah-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-temp_TestEpNormRet_halfcheetah_medium-replay.png}
\caption{HalfCheetah-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-temp_TestEpNormRet_halfcheetah_medium-expert.png}
\caption{HalfCheetah-medium-expert}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-temp_TestEpNormRet_ant_medium.png}
\caption{Ant-medium}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-temp_TestEpNormRet_ant_medium-replay.png}
\caption{Ant-medium-replay}
\end{subfigure}
\begin{subfigure}[t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{figure-curves/ind-dt-ftratio-temp_TestEpNormRet_ant_medium-expert.png}
\caption{Ant-medium-expert}
\end{subfigure}

\caption{Ablations of state, MC step and temperature against finetuning updates for individual datasets.}
\label{fig:dt-learning-curves-agg-ftratio-temp}
\end{figure}


% DT, DT+wiki, DT+MC
% best 
\begin{table*}[htb]
 \settablefontsize
 \settablecolsep
	\caption{Best test score for DT, DT with Wikipedia pre-training, and DT with MC pre-training (DT+Synthetic). The synthetic data is generated from a one-step MC with a state space size of 100, and temperature value of 1 (default values). }
	\label{table:dt-main-best}
	\begin{center}\begin{tabular}{lccccccc}
Best vs. Pre-trained Feature Difference & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
halfcheetah-medium-expert & 0.60  & 7.23  & 0.25  & \textbf{0.18}  & 0.50  & 0.68 \\
hopper-medium-expert & 0.57  & 9.11  & 0.27  & \textbf{0.17}  & 1.01  & 0.87 \\
walker2d-medium-expert & 0.62  & 7.98  & 0.24  & \textbf{0.16}  & 0.60  & 0.55 \\
ant-medium-expert & 0.81  & 7.69  & 0.37  & \textbf{0.26}  & 1.48  & 1.34 \\
halfcheetah-medium & 0.60  & 7.71  & 0.25  & \textbf{0.18}  & 0.77  & 0.66 \\
hopper-medium & 0.50  & 8.60  & 0.24  & \textbf{0.16}  & 1.21  & 0.93 \\
walker2d-medium & 0.53  & 7.64  & 0.26  & \textbf{0.18}  & 0.95  & 0.93 \\
ant-medium & 0.73  & 8.28  & 0.38  & \textbf{0.27}  & 1.78  & 1.13 \\
halfcheetah-medium-replay & 0.52  & 7.94  & 0.31  & \textbf{0.24}  & 0.83  & 0.96 \\
hopper-medium-replay & 0.44  & 9.09  & 0.34  & \textbf{0.19}  & 1.31  & 1.22 \\
walker2d-medium-replay & 0.58  & 7.37  & 0.31  & \textbf{0.21}  & 1.42  & 1.37 \\
ant-medium-replay & 0.85  & 7.45  & 0.41  & \textbf{0.30}  & 1.89  & 1.60 \\
                \hline 
Average (All Settings) & 0.61  & 8.01  & 0.30  & \textbf{0.21}  & 1.15  & 1.02 \\



Final vs. Pre-trained Feature Difference & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
halfcheetah-medium-expert & 0.76  & 8.23  & 0.30  & \textbf{0.25}  & 0.90  & 0.91 \\
hopper-medium-expert & 0.65  & 9.43  & 0.30  & \textbf{0.21}  & 1.18  & 1.09 \\
walker2d-medium-expert & 0.69  & 8.63  & 0.29  & \textbf{0.22}  & 1.06  & 0.93 \\
ant-medium-expert & 0.87  & 7.76  & 0.38  & \textbf{0.30}  & 1.66  & 1.45 \\
halfcheetah-medium & 0.73  & 8.65  & 0.32  & \textbf{0.24}  & 1.01  & 1.02 \\
hopper-medium & 0.62  & 9.78  & 0.31  & \textbf{0.21}  & 1.38  & 1.13 \\
walker2d-medium & 0.70  & 8.49  & 0.32  & \textbf{0.24}  & 1.18  & 1.07 \\
ant-medium & 0.86  & 8.34  & 0.42  & \textbf{0.31}  & 1.98  & 1.59 \\
halfcheetah-medium-replay & 0.58  & 8.34  & 0.34  & \textbf{0.28}  & 1.21  & 1.17 \\
hopper-medium-replay & 0.50  & 9.38  & 0.36  & \textbf{0.24}  & 1.79  & 1.56 \\
walker2d-medium-replay & 0.67  & 7.81  & 0.37  & \textbf{0.27}  & 1.70  & 1.65 \\
ant-medium-replay & 0.92  & 7.83  & 0.43  & \textbf{0.33}  & 1.98  & 1.69 \\
                \hline 
Average (All Settings) & 0.71  & 8.56  & 0.35  & \textbf{0.26}  & 1.42  & 1.27 \\



Best vs. Pre-trained Feature Similarity & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
halfcheetah-medium-expert & 0.72  & 0.46  & 0.78  & \textbf{0.83}  & \textbf{0.85}  & 0.81 \\
hopper-medium-expert & 0.72  & 0.33  & 0.75  & \textbf{0.83}  & 0.70  & 0.74 \\
walker2d-medium-expert & 0.70  & 0.41  & 0.78  & \textbf{0.85}  & \textbf{0.82}  & \textbf{0.84} \\
ant-medium-expert & 0.60  & 0.36  & 0.65  & \textbf{0.73}  & 0.55  & 0.61 \\
halfcheetah-medium & 0.72  & 0.42  & 0.77  & \textbf{0.81}  & \textbf{0.77}  & \textbf{0.81} \\
hopper-medium & 0.74  & 0.37  & 0.77  & \textbf{0.83}  & 0.63  & 0.72 \\
walker2d-medium & 0.74  & 0.43  & 0.75  & \textbf{0.83}  & 0.71  & 0.73 \\
ant-medium & 0.64  & 0.35  & 0.64  & \textbf{0.73}  & 0.46  & 0.68 \\
halfcheetah-medium-replay & \textbf{0.76}  & 0.39  & 0.71  & \textbf{0.76}  & \textbf{0.76}  & 0.72 \\
hopper-medium-replay & \textbf{0.74}  & 0.30  & 0.65  & \textbf{0.76}  & 0.57  & 0.61 \\
walker2d-medium-replay & 0.69  & 0.38  & 0.68  & \textbf{0.77}  & 0.54  & 0.57 \\
ant-medium-replay & 0.54  & 0.34  & 0.59  & \textbf{0.74}  & 0.41  & 0.52 \\
                \hline 
Average (All Settings) & 0.69  & 0.38  & 0.71  & \textbf{0.79}  & 0.65  & 0.70 \\



Final vs. Pre-trained Feature similarity & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
halfcheetah-medium-expert & 0.64  & 0.38  & \textbf{0.72}  & \textbf{0.74}  & \textbf{0.73}  & \textbf{0.74} \\
hopper-medium-expert & 0.68  & 0.31  & 0.72  & \textbf{0.78}  & 0.64  & 0.68 \\
walker2d-medium-expert & 0.67  & 0.35  & 0.72  & \textbf{0.78}  & 0.68  & 0.73 \\
ant-medium-expert & 0.57  & 0.35  & 0.63  & \textbf{0.68}  & 0.49  & 0.58 \\
halfcheetah-medium & 0.65  & 0.35  & 0.70  & \textbf{0.75}  & 0.70  & 0.71 \\
hopper-medium & 0.68  & 0.28  & 0.70  & \textbf{0.79}  & 0.57  & 0.66 \\
walker2d-medium & 0.66  & 0.35  & 0.70  & \textbf{0.76}  & 0.64  & 0.69 \\
ant-medium & 0.57  & 0.32  & 0.59  & \textbf{0.68}  & 0.40  & 0.54 \\
halfcheetah-medium-replay & \textbf{0.73}  & 0.36  & 0.67  & \textbf{0.70}  & 0.63  & 0.65 \\
hopper-medium-replay & \textbf{0.72}  & 0.28  & 0.62  & \textbf{0.69}  & 0.42  & 0.51 \\
walker2d-medium-replay & 0.64  & 0.33  & 0.61  & \textbf{0.69}  & 0.44  & 0.47 \\
ant-medium-replay & 0.49  & 0.29  & 0.55  & \textbf{0.70}  & 0.38  & 0.49 \\
                \hline 
Average (All Settings) & 0.64  & 0.33  & 0.66  & \textbf{0.73}  & 0.56  & 0.62 \\

\end{tabular}\end{center}\end{table*}
% DT, DT+wiki, DT+MC
% best 
\begin{table*}[htb]
 \settablefontsize
 \settablecolsep
	\caption{Best test score for DT, DT with Wikipedia pre-training, and DT with MC pre-training (DT+Synthetic). The synthetic data is generated from a one-step MC with a state space size of 100, and temperature value of 1 (default values). }
	\label{table:dt-main-best}
	\begin{center}\begin{tabular}{lccccccc}
Best vs. Pre-trained Weight Difference & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
halfcheetah-medium-expert & 1.3E-03  & 8.0E-04  & 7.9E-04  & 6.0E-04  & \textbf{4.2E-04}  & 6.2E-04 \\
hopper-medium-expert & 1.4E-03  & 1.1E-03  & 1.0E-03  & 6.7E-04  & 6.6E-04  & \textbf{6.0E-04} \\
walker2d-medium-expert & 1.6E-03  & 9.0E-04  & 8.3E-04  & 5.8E-04  & \textbf{4.5E-04}  & \textbf{4.6E-04} \\
ant-medium-expert & 2.0E-03  & 1.6E-03  & 1.3E-03  & 9.0E-04  & \textbf{8.0E-04}  & 9.3E-04 \\
halfcheetah-medium & 1.3E-03  & 7.9E-04  & 6.6E-04  & 6.0E-04  & 5.9E-04  & \textbf{4.5E-04} \\
hopper-medium & 1.1E-03  & 7.2E-04  & 6.9E-04  & \textbf{6.1E-04}  & \textbf{6.2E-04}  & \textbf{5.9E-04} \\
walker2d-medium & 1.1E-03  & 6.7E-04  & 7.9E-04  & \textbf{6.2E-04}  & \textbf{6.2E-04}  & 6.5E-04 \\
ant-medium & 1.5E-03  & 1.2E-03  & 8.6E-04  & 8.2E-04  & 6.3E-04  & \textbf{4.9E-04} \\
halfcheetah-medium-replay & 1.9E-03  & 1.3E-03  & 1.1E-03  & 7.9E-04  & \textbf{5.9E-04}  & 7.6E-04 \\
hopper-medium-replay & 1.6E-03  & 1.3E-03  & 1.3E-03  & 7.9E-04  & \textbf{6.0E-04}  & 7.1E-04 \\
walker2d-medium-replay & 1.8E-03  & 1.2E-03  & 1.0E-03  & 8.6E-04  & 9.2E-04  & \textbf{8.1E-04} \\
ant-medium-replay & 2.1E-03  & 1.5E-03  & 1.3E-03  & 1.1E-03  & \textbf{9.9E-04}  & \textbf{9.8E-04} \\
                \hline 
Average (All Settings) & 1.5E-03  & 1.1E-03  & 9.7E-04  & 7.4E-04  & \textbf{6.6E-04}  & \textbf{6.7E-04} \\



Final vs. Pre-trained Weight Difference & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
halfcheetah-medium-expert & 2.0E-03  & 1.5E-03  & 1.3E-03  & 1.1E-03  & \textbf{8.9E-04}  & \textbf{8.9E-04} \\
hopper-medium-expert & 1.8E-03  & 1.6E-03  & 1.3E-03  & 9.7E-04  & \textbf{8.4E-04}  & \textbf{8.1E-04} \\
walker2d-medium-expert & 2.0E-03  & 1.6E-03  & 1.4E-03  & 1.1E-03  & 9.0E-04  & \textbf{8.5E-04} \\
ant-medium-expert & 2.3E-03  & 1.9E-03  & 1.6E-03  & 1.2E-03  & \textbf{1.1E-03}  & \textbf{1.1E-03} \\
halfcheetah-medium & 1.9E-03  & 1.4E-03  & 1.2E-03  & 1.0E-03  & \textbf{8.5E-04}  & \textbf{8.3E-04} \\
hopper-medium & 1.6E-03  & 1.5E-03  & 1.2E-03  & 9.3E-04  & 7.9E-04  & \textbf{7.4E-04} \\
walker2d-medium & 1.9E-03  & 1.5E-03  & 1.3E-03  & 1.1E-03  & 8.7E-04  & \textbf{8.2E-04} \\
ant-medium & 2.2E-03  & 1.7E-03  & 1.4E-03  & 1.1E-03  & \textbf{8.6E-04}  & \textbf{8.4E-04} \\
halfcheetah-medium-replay & 2.4E-03  & 1.7E-03  & 1.5E-03  & 1.2E-03  & \textbf{1.0E-03}  & \textbf{9.9E-04} \\
hopper-medium-replay & 2.1E-03  & 1.8E-03  & 1.5E-03  & 1.2E-03  & \textbf{1.1E-03}  & \textbf{1.1E-03} \\
walker2d-medium-replay & 2.4E-03  & 2.0E-03  & 1.6E-03  & 1.4E-03  & 1.3E-03  & \textbf{1.2E-03} \\
ant-medium-replay & 2.6E-03  & 2.1E-03  & 1.7E-03  & 1.4E-03  & 1.2E-03  & \textbf{1.1E-03} \\
                \hline 
Average (All Settings) & 2.1E-03  & 1.7E-03  & 1.4E-03  & 1.1E-03  & \textbf{9.7E-04}  & \textbf{9.3E-04} \\



Best vs. Pre-trained Weight Similarity & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
halfcheetah-medium-expert & 0.79  & \textbf{0.92}  & 0.85  & 0.87  & \textbf{0.90}  & \textbf{0.88} \\
hopper-medium-expert & 0.78  & \textbf{0.89}  & 0.82  & \textbf{0.85}  & \textbf{0.86}  & \textbf{0.87} \\
walker2d-medium-expert & 0.76  & \textbf{0.91}  & 0.85  & \textbf{0.87}  & \textbf{0.90}  & \textbf{0.90} \\
ant-medium-expert & 0.73  & \textbf{0.85}  & 0.77  & \textbf{0.82}  & \textbf{0.84}  & \textbf{0.82} \\
halfcheetah-medium & 0.79  & \textbf{0.92}  & 0.87  & 0.86  & 0.87  & \textbf{0.90} \\
hopper-medium & 0.81  & \textbf{0.93}  & 0.87  & 0.86  & 0.86  & 0.87 \\
walker2d-medium & 0.82  & \textbf{0.93}  & 0.85  & 0.86  & 0.86  & 0.86 \\
ant-medium & 0.77  & \textbf{0.89}  & 0.84  & 0.82  & \textbf{0.86}  & \textbf{0.90} \\
halfcheetah-medium-replay & 0.75  & \textbf{0.88}  & 0.80  & 0.83  & \textbf{0.87}  & \textbf{0.85} \\
hopper-medium-replay & 0.77  & \textbf{0.88}  & 0.79  & \textbf{0.83}  & \textbf{0.87}  & \textbf{0.85} \\
walker2d-medium-replay & 0.76  & \textbf{0.88}  & 0.83  & 0.83  & 0.83  & \textbf{0.84} \\
ant-medium-replay & 0.74  & \textbf{0.86}  & 0.79  & 0.79  & 0.81  & 0.82 \\
                \hline 
Average (All Settings) & 0.77  & \textbf{0.89}  & 0.83  & 0.84  & \textbf{0.86}  & \textbf{0.86} \\



Final vs. Pre-trained Weight Similarity & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
halfcheetah-medium-expert & 0.72  & \textbf{0.85}  & 0.77  & 0.78  & \textbf{0.82}  & \textbf{0.83} \\
hopper-medium-expert & 0.74  & \textbf{0.85}  & 0.78  & 0.79  & \textbf{0.83}  & \textbf{0.84} \\
walker2d-medium-expert & 0.73  & \textbf{0.85}  & 0.77  & 0.78  & \textbf{0.82}  & \textbf{0.83} \\
ant-medium-expert & 0.70  & \textbf{0.83}  & 0.74  & 0.76  & \textbf{0.80}  & \textbf{0.80} \\
halfcheetah-medium & 0.73  & \textbf{0.86}  & 0.78  & 0.78  & \textbf{0.82}  & \textbf{0.84} \\
hopper-medium & 0.76  & \textbf{0.86}  & 0.79  & 0.80  & \textbf{0.83}  & \textbf{0.85} \\
walker2d-medium & 0.73  & \textbf{0.85}  & 0.78  & 0.78  & \textbf{0.82}  & \textbf{0.83} \\
ant-medium & 0.71  & \textbf{0.84}  & 0.76  & 0.77  & \textbf{0.82}  & \textbf{0.84} \\
halfcheetah-medium-replay & 0.71  & \textbf{0.83}  & 0.73  & 0.76  & \textbf{0.80}  & \textbf{0.80} \\
hopper-medium-replay & 0.73  & \textbf{0.84}  & 0.76  & 0.77  & 0.79  & \textbf{0.80} \\
walker2d-medium-replay & 0.71  & \textbf{0.82}  & 0.74  & 0.75  & 0.78  & \textbf{0.79} \\
ant-medium-replay & 0.70  & \textbf{0.81}  & 0.73  & 0.74  & \textbf{0.78}  & \textbf{0.80} \\
                \hline 
Average (All Settings) & 0.72  & \textbf{0.84}  & 0.76  & 0.77  & \textbf{0.81}  & \textbf{0.82} \\
\end{tabular}\end{center}\end{table*}

% DT, DT+wiki, DT+MC
% best 
\begin{table*}[htb]
 \settablefontsize
 \settablecolsep
	\caption{Best test score for DT, DT with Wikipedia pre-training, and DT with MC pre-training (DT+Synthetic). The synthetic data is generated from a one-step MC with a state space size of 100, and temperature value of 1 (default values). }
	\label{table:dt-main-best}
	\begin{center}\begin{tabular}{lccccccc}
Best vs. Random Init. Feature Difference & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
halfcheetah-medium-expert & \textbf{0.60}  & 6.58  & 1.50  & 1.52  & 2.66  & 2.75 \\
hopper-medium-expert & \textbf{0.57}  & 7.14  & 1.49  & 1.30  & 2.68  & 2.71 \\
walker2d-medium-expert & \textbf{0.62}  & 6.49  & 1.49  & 1.32  & 2.67  & 2.76 \\
ant-medium-expert & \textbf{0.81}  & 4.66  & 1.44  & 1.19  & 2.56  & 2.62 \\
halfcheetah-medium & \textbf{0.60}  & 6.54  & 1.51  & 1.35  & 2.62  & 2.77 \\
hopper-medium & \textbf{0.50}  & 7.17  & 1.48  & 1.24  & 2.62  & 2.68 \\
walker2d-medium & \textbf{0.53}  & 6.50  & 1.49  & 1.25  & 2.62  & 2.69 \\
ant-medium & \textbf{0.73}  & 5.11  & 1.48  & 1.13  & 2.57  & 2.67 \\
halfcheetah-medium-replay & \textbf{0.52}  & 6.30  & 1.46  & 1.42  & 2.63  & 2.65 \\
hopper-medium-replay & \textbf{0.44}  & 6.86  & 1.42  & 1.20  & 2.55  & 2.60 \\
walker2d-medium-replay & \textbf{0.58}  & 4.94  & 1.43  & 1.20  & 2.40  & 2.53 \\
ant-medium-replay & \textbf{0.85}  & 3.59  & 1.40  & 1.09  & 2.48  & 2.57 \\
                \hline 
Average (All Settings) & \textbf{0.61}  & 5.99  & 1.47  & 1.27  & 2.59  & 2.67 \\



Final vs. Random Init. Feature Difference & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
halfcheetah-medium-expert & \textbf{0.76}  & 6.52  & 1.45  & 1.39  & 2.59  & 2.69 \\
hopper-medium-expert & \textbf{0.65}  & 7.05  & 1.46  & 1.23  & 2.66  & 2.68 \\
walker2d-medium-expert & \textbf{0.69}  & 6.34  & 1.44  & 1.19  & 2.57  & 2.70 \\
ant-medium-expert & \textbf{0.87}  & 4.57  & 1.42  & 1.16  & 2.51  & 2.59 \\
halfcheetah-medium & \textbf{0.73}  & 6.48  & 1.45  & 1.23  & 2.58  & 2.69 \\
hopper-medium & \textbf{0.62}  & 7.23  & 1.45  & 1.15  & 2.61  & 2.67 \\
walker2d-medium & \textbf{0.70}  & 6.15  & 1.44  & 1.17  & 2.57  & 2.66 \\
ant-medium & \textbf{0.86}  & 4.84  & 1.43  & 1.11  & 2.52  & 2.62 \\
halfcheetah-medium-replay & \textbf{0.58}  & 6.24  & 1.40  & 1.37  & 2.49  & 2.57 \\
hopper-medium-replay & \textbf{0.50}  & 6.83  & 1.40  & 1.15  & 2.48  & 2.55 \\
walker2d-medium-replay & \textbf{0.67}  & 4.90  & 1.36  & 1.13  & 2.32  & 2.43 \\
ant-medium-replay & \textbf{0.92}  & 3.64  & 1.34  & 1.07  & 2.42  & 2.53 \\
                \hline 
Average (All Settings) & \textbf{0.71}  & 5.90  & 1.42  & 1.20  & 2.53  & 2.62 \\



Best vs. Random Init. Feature Similarity & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
halfcheetah-medium-expert & \textbf{0.72}  & 7.3E-03  & 2.2E-03  & 2.2E-03  & 1.2E-02  & -1.5E-02 \\
hopper-medium-expert & \textbf{0.72}  & 2.9E-03  & 4.6E-03  & 1.0E-02  & -1.3E-02  & -1.3E-03 \\
walker2d-medium-expert & \textbf{0.70}  & 5.9E-03  & 3.6E-03  & 6.0E-03  & 5.8E-03  & -1.7E-02 \\
ant-medium-expert & \textbf{0.60}  & 3.1E-03  & -7.4E-03  & 7.4E-04  & 8.9E-03  & 1.4E-02 \\
halfcheetah-medium & \textbf{0.72}  & 7.8E-03  & -3.4E-03  & -2.9E-03  & 1.3E-02  & -1.5E-02 \\
hopper-medium & \textbf{0.74}  & 3.8E-03  & 7.1E-03  & 1.2E-02  & -6.4E-03  & -1.0E-03 \\
walker2d-medium & \textbf{0.74}  & 5.0E-03  & 1.8E-03  & 5.4E-03  & 3.4E-03  & -5.3E-03 \\
ant-medium & \textbf{0.64}  & 3.5E-03  & -7.3E-03  & -2.5E-03  & 3.2E-03  & 1.4E-02 \\
halfcheetah-medium-replay & \textbf{0.76}  & 3.8E-03  & -1.0E-03  & -1.3E-03  & 1.4E-02  & 4.7E-04 \\
hopper-medium-replay & \textbf{0.74}  & -2.0E-03  & 8.1E-03  & 1.6E-02  & 1.1E-03  & 1.6E-03 \\
walker2d-medium-replay & \textbf{0.69}  & 4.9E-03  & 6.1E-05  & -3.6E-03  & 2.0E-02  & -5.8E-03 \\
ant-medium-replay & \textbf{0.54}  & 2.0E-03  & -5.9E-03  & -5.3E-03  & 3.3E-03  & 3.2E-03 \\
                \hline 
Average (All Settings) & \textbf{0.69}  & 4.0E-03  & 2.1E-04  & 3.1E-03  & 5.4E-03  & -2.3E-03 \\



Final vs. Random Init. Feature similarity & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
halfcheetah-medium-expert & \textbf{0.64}  & 5.4E-03  & 2.1E-03  & 3.3E-03  & 7.1E-03  & -1.3E-02 \\
hopper-medium-expert & \textbf{0.68}  & 2.4E-03  & 4.8E-03  & 1.1E-02  & -1.5E-02  & -2.2E-03 \\
walker2d-medium-expert & \textbf{0.67}  & 4.7E-03  & 3.6E-03  & 7.7E-03  & 7.1E-03  & -2.0E-02 \\
ant-medium-expert & \textbf{0.57}  & 2.9E-03  & -7.0E-03  & 1.4E-03  & 7.0E-03  & 1.4E-02 \\
halfcheetah-medium & \textbf{0.65}  & 5.6E-03  & -4.3E-03  & -1.7E-03  & 1.2E-02  & -1.1E-02 \\
hopper-medium & \textbf{0.68}  & 6.6E-04  & 4.4E-03  & 1.3E-02  & -1.0E-02  & -2.5E-03 \\
walker2d-medium & \textbf{0.66}  & 4.1E-03  & 2.3E-03  & 6.6E-03  & 8.0E-03  & -5.7E-03 \\
ant-medium & \textbf{0.57}  & 3.3E-03  & -7.9E-03  & -5.3E-03  & 1.6E-03  & 1.3E-02 \\
halfcheetah-medium-replay & \textbf{0.73}  & 1.9E-03  & 2.0E-04  & -9.5E-04  & 1.1E-02  & -8.5E-04 \\
hopper-medium-replay & \textbf{0.72}  & -1.7E-03  & 7.1E-03  & 1.4E-02  & -1.8E-03  & 1.5E-03 \\
walker2d-medium-replay & \textbf{0.64}  & 3.8E-03  & 1.7E-03  & -1.4E-03  & 1.7E-02  & -6.4E-03 \\
ant-medium-replay & \textbf{0.49}  & 1.5E-03  & -6.6E-03  & -4.7E-03  & 3.1E-03  & 2.3E-03 \\
                \hline 
Average (All Settings) & \textbf{0.64}  & 2.9E-03  & 5.2E-05  & 3.6E-03  & 3.9E-03  & -2.6E-03 \\


\end{tabular}\end{center}\end{table*}

% DT, DT+wiki, DT+MC
% best 
\begin{table*}[htb]
 \settablefontsize
 \settablecolsep
	\caption{Best test score for DT, DT with Wikipedia pre-training, and DT with MC pre-training (DT+Synthetic). The synthetic data is generated from a one-step MC with a state space size of 100, and temperature value of 1 (default values). }
	\label{table:dt-main-best}
	\begin{center}\begin{tabular}{lccccccc}
Best vs. Random Init. Weight Difference & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
halfcheetah-medium-expert & 1.3E-03  & 3.0E-03  & 1.8E-03  & 1.2E-03  & \textbf{9.0E-04}  & 1.3E-03 \\
hopper-medium-expert & 1.4E-03  & 3.4E-03  & 2.0E-03  & 1.3E-03  & \textbf{1.1E-03}  & 1.2E-03 \\
walker2d-medium-expert & 1.6E-03  & 3.2E-03  & 1.8E-03  & 1.2E-03  & \textbf{9.4E-04}  & 1.1E-03 \\
ant-medium-expert & 2.0E-03  & 3.6E-03  & 2.2E-03  & 1.5E-03  & \textbf{1.3E-03}  & 1.5E-03 \\
halfcheetah-medium & 1.3E-03  & 3.0E-03  & 1.7E-03  & 1.2E-03  & \textbf{1.1E-03}  & 1.1E-03 \\
hopper-medium & \textbf{1.1E-03}  & 3.1E-03  & 1.7E-03  & 1.2E-03  & \textbf{1.1E-03}  & 1.2E-03 \\
walker2d-medium & \textbf{1.1E-03}  & 3.0E-03  & 1.8E-03  & 1.2E-03  & \textbf{1.1E-03}  & 1.2E-03 \\
ant-medium & 1.5E-03  & 3.3E-03  & 1.8E-03  & 1.4E-03  & \textbf{1.1E-03}  & 1.2E-03 \\
halfcheetah-medium-replay & 1.9E-03  & 3.4E-03  & 2.0E-03  & 1.4E-03  & \textbf{1.1E-03}  & 1.3E-03 \\
hopper-medium-replay & 1.6E-03  & 3.6E-03  & 2.2E-03  & 1.4E-03  & \textbf{1.1E-03}  & 1.3E-03 \\
walker2d-medium-replay & 1.8E-03  & 3.5E-03  & 2.0E-03  & 1.5E-03  & \textbf{1.4E-03}  & \textbf{1.4E-03} \\
ant-medium-replay & 2.1E-03  & 3.6E-03  & 2.2E-03  & 1.7E-03  & \textbf{1.5E-03}  & 1.6E-03 \\
                \hline 
Average (All Settings) & 1.5E-03  & 3.3E-03  & 1.9E-03  & 1.3E-03  & \textbf{1.1E-03}  & 1.3E-03 \\



Final vs. Random Init. Weight Difference & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
halfcheetah-medium-expert & 2.0E-03  & 3.6E-03  & 2.2E-03  & 1.6E-03  & \textbf{1.4E-03}  & 1.5E-03 \\
hopper-medium-expert & 1.8E-03  & 3.8E-03  & 2.3E-03  & 1.5E-03  & \textbf{1.3E-03}  & 1.4E-03 \\
walker2d-medium-expert & 2.0E-03  & 3.7E-03  & 2.3E-03  & 1.7E-03  & \textbf{1.4E-03}  & \textbf{1.4E-03} \\
ant-medium-expert & 2.3E-03  & 3.8E-03  & 2.4E-03  & 1.8E-03  & \textbf{1.5E-03}  & 1.6E-03 \\
halfcheetah-medium & 1.9E-03  & 3.5E-03  & 2.1E-03  & 1.6E-03  & \textbf{1.3E-03}  & 1.5E-03 \\
hopper-medium & 1.6E-03  & 3.7E-03  & 2.1E-03  & 1.5E-03  & \textbf{1.3E-03}  & 1.3E-03 \\
walker2d-medium & 1.9E-03  & 3.7E-03  & 2.2E-03  & 1.7E-03  & \textbf{1.3E-03}  & \textbf{1.4E-03} \\
ant-medium & 2.2E-03  & 3.7E-03  & 2.2E-03  & 1.6E-03  & \textbf{1.3E-03}  & 1.5E-03 \\
halfcheetah-medium-replay & 2.4E-03  & 3.7E-03  & 2.3E-03  & 1.7E-03  & \textbf{1.5E-03}  & 1.5E-03 \\
hopper-medium-replay & 2.1E-03  & 4.0E-03  & 2.4E-03  & 1.8E-03  & \textbf{1.6E-03}  & \textbf{1.6E-03} \\
walker2d-medium-replay & 2.4E-03  & 4.1E-03  & 2.5E-03  & 2.0E-03  & \textbf{1.7E-03}  & \textbf{1.7E-03} \\
ant-medium-replay & 2.6E-03  & 4.0E-03  & 2.5E-03  & 2.0E-03  & \textbf{1.7E-03}  & \textbf{1.7E-03} \\
                \hline 
Average (All Settings) & 2.1E-03  & 3.8E-03  & 2.3E-03  & 1.7E-03  & \textbf{1.4E-03}  & 1.5E-03 \\



Best vs. Random Init. Weight Similarity & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
halfcheetah-medium-expert & \textbf{0.79}  & 0.63  & 0.63  & 0.72  & \textbf{0.78}  & 0.72 \\
hopper-medium-expert & \textbf{0.78}  & 0.61  & 0.61  & 0.71  & \textbf{0.74}  & 0.73 \\
walker2d-medium-expert & \textbf{0.76}  & 0.63  & 0.63  & 0.72  & \textbf{0.78}  & \textbf{0.75} \\
ant-medium-expert & \textbf{0.73}  & 0.60  & 0.60  & 0.69  & \textbf{0.73}  & 0.70 \\
halfcheetah-medium & \textbf{0.79}  & 0.63  & 0.65  & 0.72  & 0.75  & 0.74 \\
hopper-medium & \textbf{0.81}  & 0.63  & 0.64  & 0.71  & 0.74  & 0.73 \\
walker2d-medium & \textbf{0.82}  & 0.64  & 0.63  & 0.71  & 0.75  & 0.72 \\
ant-medium & \textbf{0.77}  & 0.62  & 0.64  & 0.69  & \textbf{0.75}  & \textbf{0.74} \\
halfcheetah-medium-replay & \textbf{0.75}  & 0.62  & 0.61  & 0.69  & \textbf{0.75}  & 0.71 \\
hopper-medium-replay & \textbf{0.77}  & 0.60  & 0.59  & 0.69  & \textbf{0.75}  & 0.72 \\
walker2d-medium-replay & \textbf{0.76}  & 0.61  & 0.62  & 0.69  & 0.71  & 0.71 \\
ant-medium-replay & \textbf{0.74}  & 0.60  & 0.60  & 0.66  & \textbf{0.70}  & 0.69 \\
                \hline 
Average (All Settings) & \textbf{0.77}  & 0.62  & 0.62  & 0.70  & \textbf{0.75}  & 0.72 \\



Final vs. Random Init. Weight Similarity & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
halfcheetah-medium-expert & \textbf{0.72}  & 0.60  & 0.58  & 0.66  & \textbf{0.71}  & \textbf{0.69} \\
hopper-medium-expert & \textbf{0.74}  & 0.59  & 0.58  & 0.66  & \textbf{0.72}  & 0.70 \\
walker2d-medium-expert & \textbf{0.73}  & 0.60  & 0.58  & 0.65  & \textbf{0.71}  & \textbf{0.70} \\
ant-medium-expert & \textbf{0.70}  & 0.59  & 0.58  & 0.64  & \textbf{0.70}  & \textbf{0.68} \\
halfcheetah-medium & \textbf{0.73}  & 0.60  & 0.59  & 0.65  & \textbf{0.71}  & 0.69 \\
hopper-medium & \textbf{0.76}  & 0.59  & 0.59  & 0.66  & 0.72  & 0.70 \\
walker2d-medium & \textbf{0.73}  & 0.60  & 0.59  & 0.65  & \textbf{0.71}  & \textbf{0.70} \\
ant-medium & \textbf{0.71}  & 0.59  & 0.59  & 0.65  & \textbf{0.72}  & \textbf{0.69} \\
halfcheetah-medium-replay & \textbf{0.71}  & 0.60  & 0.57  & 0.64  & \textbf{0.70}  & \textbf{0.68} \\
hopper-medium-replay & \textbf{0.73}  & 0.58  & 0.57  & 0.64  & 0.68  & 0.68 \\
walker2d-medium-replay & \textbf{0.71}  & 0.58  & 0.57  & 0.62  & 0.67  & 0.67 \\
ant-medium-replay & \textbf{0.70}  & 0.58  & 0.57  & 0.62  & \textbf{0.68}  & \textbf{0.67} \\
                \hline 
Average (All Settings) & \textbf{0.72}  & 0.59  & 0.58  & 0.65  & \textbf{0.70}  & \textbf{0.69} \\
\end{tabular}\end{center}\end{table*}
\end{comment}


\begin{comment}
    \begin{table*}[htb]
 \settablefontsize
 \settablecolsep
	\caption{Best test score for DT, DT with Wikipedia pre-training, and DT with MC pre-training (DT+Synthetic). The synthetic data is generated from a one-step MC with a state space size of 100, and temperature value of 1 (default values). }
	\label{table:dt-main-best}
	\begin{center}\begin{tabular}{lccccccc}
Average (All Settings) & DT & DT+Wiki & DT+Synthetic & DT+IID & DT+Identity & DT+Mapping \\
                \hline 
%FT vs. PT Feature Diff. & -  & 8.56  & 0.35  & \textbf{0.26}  & 1.42  & 1.27 \\
%FT vs. RI Feature Diff. & \textbf{0.71}  & 5.90  & 1.42  & 1.20  & 2.53  & %2.62 \\
%                \hline 
FT vs. PT Feature Sim. & -  & 0.33  & 0.66  & \textbf{0.73}  & 0.56  & 0.62 \\
FT vs. RI Feature Sim. & \textbf{0.64}  & 2.9E-03  & 5.2E-05  & 3.6E-03  & 3.9E-03  & -2.6E-03 \\
                \hline 
%FT vs. PT Weight Diff. & -  & 1.7E-03  & 1.4E-03  & 1.1E-03  & \textbf{9.7E-04}  & \textbf{9.3E-04} \\
%FT vs. RI Weight Diff. & 2.1E-03  & 3.8E-03  & 2.3E-03  & 1.7E-03  & \textbf{1.4E-03}  & 1.5E-03 \\
%                \hline 
FT vs. PT Weight Sim. & -  & \textbf{0.84}  & 0.76  & 0.77  & \textbf{0.81}  & \textbf{0.82} \\
FT vs. RI Weight Sim. & \textbf{0.72}  & 0.59  & 0.58  & 0.65  & \textbf{0.70}  & \textbf{0.69} \\
\end{tabular}\end{center}\end{table*}

\end{comment}

==> tables/dt_table_more_baseline_best.tex <==
\begin{table*}[htb]
\settablefontsize
\settablecolsep
	\caption{Pre-training with more updates.  Other parameters remain the default values.}
	\label{table:dt-more-updates}
	\begin{center}\begin{tabular}{lccccccc}
Best Score & DT & DT 20K more & DT 80K more & DT+Wiki & DT+Synthetic \\
                \hline 
halfcheetah-medium-expert & 66.9 $\pm$ 8.6 & 67.4 $\pm$ 9.9 & 70.3 $\pm$ 11.4 & 64.2 $\pm$ 11.5 & \textbf{72.7} $\pm$ 16.8\\
hopper-medium-expert & 106.2 $\pm$ 1.4 & 106.8 $\pm$ 4.0 & \textbf{110.6} $\pm$ 2.2 & \textbf{111.4} $\pm$ 1.5 & \textbf{111.5} $\pm$ 0.8\\
walker2d-medium-expert & \textbf{109.0} $\pm$ 0.1 & \textbf{108.6} $\pm$ 0.4 & \textbf{108.9} $\pm$ 0.3 & \textbf{109.2} $\pm$ 0.5 & \textbf{109.1} $\pm$ 0.3\\
ant-medium-expert & 127.3 $\pm$ 6.4 & 127.8 $\pm$ 5.5 & \textbf{132.1} $\pm$ 3.4 & 128.7 $\pm$ 7.0 & \textbf{131.5} $\pm$ 5.1\\
halfcheetah-medium & \textbf{43.4} $\pm$ 0.2 & \textbf{43.3} $\pm$ 0.1 & \textbf{43.6} $\pm$ 0.2 & \textbf{43.4} $\pm$ 0.2 & \textbf{43.3} $\pm$ 0.2\\
hopper-medium & 66.6 $\pm$ 2.8 & 69.2 $\pm$ 5.5 & 69.9 $\pm$ 3.4 & \textbf{70.4} $\pm$ 5.1 & \textbf{70.9} $\pm$ 4.4\\
walker2d-medium & \textbf{79.6} $\pm$ 0.4 & \textbf{79.6} $\pm$ 1.1 & \textbf{79.9} $\pm$ 1.0 & \textbf{79.3} $\pm$ 1.2 & 79.0 $\pm$ 1.2\\
ant-medium & \textbf{100.7} $\pm$ 1.3 & \textbf{100.7} $\pm$ 1.1 & \textbf{100.7} $\pm$ 1.2 & \textbf{100.6} $\pm$ 1.2 & \textbf{100.5} $\pm$ 0.8\\
halfcheetah-medium-replay & 39.8 $\pm$ 0.4 & 39.8 $\pm$ 0.5 & 40.3 $\pm$ 0.4 & \textbf{41.3} $\pm$ 0.5 & \textbf{41.5} $\pm$ 0.4\\
hopper-medium-replay & 72.2 $\pm$ 3.6 & 80.1 $\pm$ 6.4 & \textbf{84.1} $\pm$ 5.5 & 80.5 $\pm$ 5.6 & \textbf{84.8} $\pm$ 7.6\\
walker2d-medium-replay & 72.9 $\pm$ 4.7 & 74.4 $\pm$ 4.5 & \textbf{77.2} $\pm$ 2.5 & 72.9 $\pm$ 3.9 & 75.2 $\pm$ 4.0\\
ant-medium-replay & 94.5 $\pm$ 1.0 & 94.3 $\pm$ 1.5 & 94.9 $\pm$ 1.6 & 92.0 $\pm$ 2.9 & \textbf{95.9} $\pm$ 1.0\\
                \hline 
Average (All Settings) & 81.6 $\pm$ 2.6 & 82.7 $\pm$ 3.4 & \textbf{84.4} $\pm$ 2.8 & 82.8 $\pm$ 3.4 & \textbf{84.7} $\pm$ 3.6\\

\end{tabular}
\end{center}
\end{table*}

==> tables/dt_table_mroe_pretrain_best.tex <==




\begin{table*}[htb]
\settablefontsize
\settablecolsep
	\caption{Best performance for DT, DT pre-trained with Wikipedia data, DT pre-trained with Markov Chain synthetic data of default parameters, and DT pre-trained with two additional synthetic datasets: Identity Operation and Token Mapping.}
	\label{table:dt-more_pretrain}
	\begin{center}\begin{tabular}{lccccccc}

Best Score & DT & DT+Wiki &DT+Synthetic & DT+Identity & DT+Mapping\\
                \hline 
halfcheetah-medium-expert & 67.2 $\pm$ 9.1 & 64.2 $\pm$ 11.5 &  \textbf{72.7} $\pm$ 16.8 & 64.6 $\pm$ 12.1 & 71.6 $\pm$ 15.0 \\
hopper-medium-expert & 106.1 $\pm$ 4.2 & \textbf{111.4} $\pm$ 1.5 & \textbf{111.5} $\pm$ 0.8 &109.4 $\pm$ 3.1 & \textbf{111.0} $\pm$ 1.1 \\
walker2d-medium-expert & \textbf{108.6} $\pm$ 0.4 & \textbf{109.2} $\pm$ 0.5 & \textbf{109.1} $\pm$ 0.3 &109.2 $\pm$ 0.6 & \textbf{109.2} $\pm$ 0.5 \\
ant-medium-expert & 127.6 $\pm$ 4.3 & 128.7 $\pm$ 7.0 & 131.5 $\pm$ 5.1& 129.0 $\pm$ 5.2 & \textbf{133.6} $\pm$ 1.1\\
halfcheetah-medium & \textbf{43.3} $\pm$ 0.2 & \textbf{43.4} $\pm$ 0.2 & \textbf{43.3} $\pm$ 0.2& \textbf{43.4} $\pm$ 0.2 & \textbf{43.3} $\pm$ 0.3\\
hopper-medium & 68.3 $\pm$ 4.0 & \textbf{70.4} $\pm$ 5.1 &  \textbf{70.9} $\pm$ 4.4&68.9 $\pm$ 6.1 & 66.1 $\pm$ 4.0\\
walker2d-medium & 78.9 $\pm$ 1.5 & \textbf{79.3} $\pm$ 1.2 & 79.0 $\pm$ 1.2& \textbf{79.9} $\pm$ 1.4 & \textbf{79.6} $\pm$ 1.0\\
ant-medium & \textbf{100.4} $\pm$ 1.8 & \textbf{100.6} $\pm$ 1.2 & \textbf{100.5} $\pm$ 0.8& \textbf{99.7} $\pm$ 1.8 & \textbf{99.7} $\pm$ 1.8\\
halfcheetah-medium-replay & 39.9 $\pm$ 0.4 & \textbf{41.3} $\pm$ 0.5 & \textbf{41.5} $\pm$ 0.4& 41.0 $\pm$ 0.2 & \textbf{41.2} $\pm$ 0.3\\
hopper-medium-replay & 77.8 $\pm$ 7.0 & 80.5 $\pm$ 5.6 & \textbf{84.8} $\pm$ 7.6& 82.9 $\pm$ 9.7 & 80.5 $\pm$ 6.2 \\
walker2d-medium-replay & 73.9 $\pm$ 3.7 & 72.9 $\pm$ 3.9 & \textbf{75.2} $\pm$ 4.0& \textbf{74.8} $\pm$ 3.6 & 71.7 $\pm$ 4.0\\
ant-medium-replay & 92.4 $\pm$ 2.5 & 92.0 $\pm$ 2.9 & \textbf{95.9} $\pm$ 1.0& \textbf{95.0} $\pm$ 1.0 & 94.8 $\pm$ 3.0\\
                \hline 
Average (All Settings) & 82.0 $\pm$ 3.3 & 82.8 $\pm$ 3.4 & \textbf{84.7} $\pm$ 3.6& 83.2 $\pm$ 3.8 & 83.5 $\pm$ 3.2\\
 \end{tabular}
\end{center}
\end{table*}

==> tables/new_cql_20seeds_best.tex <==
\begin{table*} [htb]\settablefontsize \settablecolsep
\caption{Best test score for some key experiments with 20 seeds. The number following the pretraining style indicates the total number of pretraining updates. For example, `MDP1m' means pretraining with MDP data for 1M timesteps.}
\label{table:cql-abl-ns-best}
\begin{center}{\begin{tabular}{lllllllllll}

Best & CQL & IID1m & IID100k & MDP1m & MDP100k & MDP50k & MDP25k & MDP1k & MDP1 \\
		\hline 
halfcheetah-medium-expert & 47.4 $\pm$ 6.3 & \textbf{81.2} $\pm$ 5.9 & \textbf{84.0} $\pm$ 3.8 & \textbf{82.4} $\pm$ 5.8 & \textbf{85.3} $\pm$ 3.1 & \textbf{82.0} $\pm$ 5.6 & 77.9 $\pm$ 7.1 & 58.5 $\pm$ 8.1 & 48.0 $\pm$ 3.2\\
hopper-medium-expert & \textbf{109.8} $\pm$ 3.9 & \textbf{111.5} $\pm$ 0.6 & \textbf{111.0} $\pm$ 1.2 & \textbf{111.5} $\pm$ 0.5 & \textbf{111.3} $\pm$ 1.1 & \textbf{111.3} $\pm$ 0.4 & \textbf{110.0} $\pm$ 3.0 & \textbf{110.7} $\pm$ 1.6 & \textbf{110.0} $\pm$ 2.2\\
walker2d-medium-expert & \textbf{112.9} $\pm$ 1.4 & \textbf{112.5} $\pm$ 1.3 & \textbf{113.4} $\pm$ 1.8 & \textbf{112.2} $\pm$ 0.6 & \textbf{112.2} $\pm$ 0.8 & \textbf{113.0} $\pm$ 1.5 & \textbf{113.3} $\pm$ 1.3 & \textbf{113.1} $\pm$ 1.0 & \textbf{113.7} $\pm$ 1.8\\
ant-medium-expert & \textbf{127.8} $\pm$ 2.0 & \textbf{131.6} $\pm$ 1.0 & \textbf{131.4} $\pm$ 1.2 & \textbf{132.1} $\pm$ 0.9 & \textbf{132.1} $\pm$ 1.1 & \textbf{132.0} $\pm$ 0.8 & \textbf{130.5} $\pm$ 0.9 & \textbf{130.5} $\pm$ 1.0 & \textbf{127.5} $\pm$ 1.1\\
halfcheetah-medium & \textbf{46.9} $\pm$ 0.2 & \textbf{47.2} $\pm$ 0.2 & \textbf{47.3} $\pm$ 0.2 & \textbf{47.2} $\pm$ 0.2 & \textbf{47.4} $\pm$ 0.2 & \textbf{47.3} $\pm$ 0.2 & \textbf{47.3} $\pm$ 0.2 & \textbf{47.3} $\pm$ 0.2 & \textbf{46.9} $\pm$ 0.2\\
hopper-medium & \textbf{87.2} $\pm$ 4.0 & \textbf{83.3} $\pm$ 2.7 & \textbf{84.5} $\pm$ 3.5 & \textbf{84.3} $\pm$ 3.0 & \textbf{84.3} $\pm$ 3.2 & \textbf{87.4} $\pm$ 3.2 & \textbf{84.0} $\pm$ 2.7 & \textbf{86.9} $\pm$ 2.6 & \textbf{87.0} $\pm$ 3.0\\
walker2d-medium & \textbf{85.7} $\pm$ 0.6 & \textbf{86.0} $\pm$ 0.5 & \textbf{86.3} $\pm$ 0.8 & \textbf{86.3} $\pm$ 0.5 & \textbf{86.2} $\pm$ 0.6 & \textbf{86.1} $\pm$ 0.4 & \textbf{85.9} $\pm$ 0.5 & \textbf{86.2} $\pm$ 0.6 & \textbf{85.9} $\pm$ 0.6\\
ant-medium & \textbf{104.2} $\pm$ 1.2 & \textbf{104.7} $\pm$ 0.7 & \textbf{104.4} $\pm$ 0.7 & \textbf{105.0} $\pm$ 0.7 & \textbf{104.7} $\pm$ 0.5 & \textbf{104.7} $\pm$ 0.5 & \textbf{104.8} $\pm$ 0.6 & \textbf{104.7} $\pm$ 0.7 & \textbf{104.1} $\pm$ 0.6\\
halfcheetah-medium-replay & \textbf{45.7} $\pm$ 0.4 & \textbf{45.4} $\pm$ 0.2 & \textbf{45.9} $\pm$ 0.3 & \textbf{45.7} $\pm$ 0.4 & \textbf{45.9} $\pm$ 0.3 & \textbf{45.7} $\pm$ 0.4 & \textbf{45.9} $\pm$ 0.3 & \textbf{45.7} $\pm$ 0.4 & \textbf{45.8} $\pm$ 0.3\\
hopper-medium-replay & \textbf{99.6} $\pm$ 1.2 & \textbf{101.3} $\pm$ 1.0 & \textbf{99.3} $\pm$ 1.2 & \textbf{100.8} $\pm$ 1.1 & \textbf{100.1} $\pm$ 1.5 & \textbf{100.2} $\pm$ 1.0 & \textbf{99.8} $\pm$ 0.9 & \textbf{100.3} $\pm$ 1.4 & \textbf{99.7} $\pm$ 1.2\\
walker2d-medium-replay & \textbf{87.7} $\pm$ 1.3 & \textbf{89.1} $\pm$ 1.0 & \textbf{89.8} $\pm$ 0.9 & \textbf{88.9} $\pm$ 1.3 & \textbf{89.2} $\pm$ 1.1 & \textbf{89.7} $\pm$ 1.0 & \textbf{89.8} $\pm$ 1.3 & \textbf{88.4} $\pm$ 1.2 & \textbf{87.6} $\pm$ 1.1\\
ant-medium-replay & \textbf{99.8} $\pm$ 1.1 & \textbf{102.1} $\pm$ 0.8 & \textbf{102.6} $\pm$ 1.1 & \textbf{102.1} $\pm$ 0.9 & \textbf{103.0} $\pm$ 1.0 & \textbf{102.6} $\pm$ 1.3 & \textbf{102.3} $\pm$ 0.8 & \textbf{102.0} $\pm$ 1.1 & \textbf{100.6} $\pm$ 1.0\\
		\hline 
Average over datasets & \textbf{87.9} $\pm$ 2.0 & \textbf{91.3} $\pm$ 1.3 & \textbf{91.7} $\pm$ 1.4 & \textbf{91.6} $\pm$ 1.3 & \textbf{91.8} $\pm$ 1.2 & \textbf{91.8} $\pm$ 1.4 & \textbf{91.0} $\pm$ 1.6 & \textbf{89.5} $\pm$ 1.7 & \textbf{88.1} $\pm$ 1.4\\

\end{tabular}}\end{center}\end{table*}



\begin{table*} [htb]\settablefontsize \settablecolsep
\caption{Best test score for some experiments with 20 seeds and the corresponding old experiments with much fewer seeds. Every two experiments is one pair indicating the old-result column followed by the new-result column (column name ends with 20). The number prefixing the pretraining style is the total number of pretraining timesteps. For example, `1mMDP20' means pretraining with MDP data for 1M timesteps averaged over 20 seeds.}
\label{table:cql-abl-ns-best}
\begin{center}{\begin{tabular}{lllllllllllllll}

Best & CQL & CQL20 & IID & IID20 & 1mMDP & 1mMDP20 \\
		\hline 
halfcheetah-medium-expert & 44.6 $\pm$ 6.4 & 47.4 $\pm$ 6.3 & 79.1 $\pm$ 5.4 & \textbf{81.2} $\pm$ 5.9 & \textbf{84.7} $\pm$ 4.2 & \textbf{82.4} $\pm$ 5.8\\
hopper-medium-expert & \textbf{106.7} $\pm$ 6.6 & \textbf{109.8} $\pm$ 3.9 & \textbf{111.5} $\pm$ 0.5 & \textbf{111.5} $\pm$ 0.6 & \textbf{111.2} $\pm$ 0.3 & \textbf{111.5} $\pm$ 0.5\\
walker2d-medium-expert & \textbf{112.1} $\pm$ 0.5 & \textbf{112.9} $\pm$ 1.4 & \textbf{114.0} $\pm$ 1.5 & \textbf{112.5} $\pm$ 1.3 & \textbf{112.4} $\pm$ 0.6 & \textbf{112.2} $\pm$ 0.6\\
ant-medium-expert & \textbf{128.7} $\pm$ 0.9 & \textbf{127.8} $\pm$ 2.0 & \textbf{129.7} $\pm$ 0.8 & \textbf{131.6} $\pm$ 1.0 & \textbf{130.6} $\pm$ 0.7 & \textbf{132.1} $\pm$ 0.9\\
halfcheetah-medium & \textbf{46.9} $\pm$ 0.1 & \textbf{46.9} $\pm$ 0.2 & \textbf{47.1} $\pm$ 0.2 & \textbf{47.2} $\pm$ 0.2 & \textbf{47.3} $\pm$ 0.1 & \textbf{47.2} $\pm$ 0.2\\
hopper-medium & \textbf{86.5} $\pm$ 4.7 & \textbf{87.2} $\pm$ 4.0 & \textbf{87.8} $\pm$ 3.4 & 83.3 $\pm$ 2.7 & \textbf{85.4} $\pm$ 1.1 & \textbf{84.3} $\pm$ 3.0\\
walker2d-medium & \textbf{85.6} $\pm$ 0.4 & \textbf{85.7} $\pm$ 0.6 & \textbf{86.2} $\pm$ 0.3 & \textbf{86.0} $\pm$ 0.5 & \textbf{86.0} $\pm$ 0.3 & \textbf{86.3} $\pm$ 0.5\\
ant-medium & \textbf{103.5} $\pm$ 0.7 & \textbf{104.2} $\pm$ 1.2 & \textbf{104.4} $\pm$ 0.9 & \textbf{104.7} $\pm$ 0.7 & \textbf{104.9} $\pm$ 0.6 & \textbf{105.0} $\pm$ 0.7\\
halfcheetah-medium-replay & \textbf{45.7} $\pm$ 0.2 & \textbf{45.7} $\pm$ 0.4 & \textbf{45.4} $\pm$ 0.2 & \textbf{45.4} $\pm$ 0.2 & \textbf{45.7} $\pm$ 0.4 & \textbf{45.7} $\pm$ 0.4\\
hopper-medium-replay & \textbf{100.2} $\pm$ 1.4 & \textbf{99.6} $\pm$ 1.2 & \textbf{100.5} $\pm$ 0.6 & \textbf{101.3} $\pm$ 1.0 & \textbf{101.0} $\pm$ 1.2 & \textbf{100.8} $\pm$ 1.1\\
walker2d-medium-replay & \textbf{88.3} $\pm$ 1.6 & \textbf{87.7} $\pm$ 1.3 & \textbf{89.3} $\pm$ 1.3 & \textbf{89.1} $\pm$ 1.0 & \textbf{89.5} $\pm$ 1.1 & \textbf{88.9} $\pm$ 1.3\\
ant-medium-replay & \textbf{99.5} $\pm$ 1.5 & \textbf{99.8} $\pm$ 1.1 & \textbf{101.8} $\pm$ 0.6 & \textbf{102.1} $\pm$ 0.8 & \textbf{102.5} $\pm$ 0.7 & \textbf{102.1} $\pm$ 0.9\\
		\hline 
Average over datasets & \textbf{87.3} $\pm$ 2.1 & \textbf{87.9} $\pm$ 2.0 & \textbf{91.4} $\pm$ 1.3 & \textbf{91.3} $\pm$ 1.3 & \textbf{91.8} $\pm$ 0.9 & \textbf{91.6} $\pm$ 1.3\\


\end{tabular}}\end{center}\end{table*}



\begin{table*} [htb]\settablefontsize \settablecolsep
\caption{Best test score for some experiments with 20 seeds and the corresponding old experiments with much fewer seeds. Every two experiments is one pair indicating the old-result column followed by the new-result column (column name ends with 20). The number prefixing the pretraining style is the total number of pretraining timesteps. For example, `1mMDP20' means pretraining with MDP data for 1M timesteps averaged over 20 seeds.}
\label{table:cql-abl-ns-best}
\begin{center}{\begin{tabular}{lllllllllllllll}

Best & 50kMDP & 50kMDP20 & 1kMDP & 1kMDP20 & 1MDP & 1MDP20 \\
		\hline 
halfcheetah-medium-expert & \textbf{82.6} $\pm$ 0.2 & \textbf{82.0} $\pm$ 5.6 & 62.6 $\pm$ 6.3 & 58.5 $\pm$ 8.1 & 56.5 $\pm$ 1.4 & 48.0 $\pm$ 3.2\\
hopper-medium-expert & \textbf{110.1} $\pm$ 1.3 & \textbf{111.3} $\pm$ 0.4 & \textbf{111.5} $\pm$ 0.9 & \textbf{110.7} $\pm$ 1.6 & \textbf{111.9} $\pm$ 0.3 & \textbf{110.0} $\pm$ 2.2\\
walker2d-medium-expert & \textbf{113.3} $\pm$ 0.4 & \textbf{113.0} $\pm$ 1.5 & \textbf{113.0} $\pm$ 0.7 & \textbf{113.1} $\pm$ 1.0 & \textbf{112.5} $\pm$ 0.5 & \textbf{113.7} $\pm$ 1.8\\
ant-medium-expert & \textbf{132.9} $\pm$ 0.9 & \textbf{132.0} $\pm$ 0.8 & \textbf{130.3} $\pm$ 1.3 & \textbf{130.5} $\pm$ 1.0 & \textbf{126.3} $\pm$ 1.4 & \textbf{127.5} $\pm$ 1.1\\
halfcheetah-medium & \textbf{47.5} $\pm$ 0.2 & \textbf{47.3} $\pm$ 0.2 & \textbf{47.2} $\pm$ 0.2 & \textbf{47.3} $\pm$ 0.2 & \textbf{46.9} $\pm$ 0.0 & \textbf{46.9} $\pm$ 0.2\\
hopper-medium & 83.9 $\pm$ 2.5 & \textbf{87.4} $\pm$ 3.2 & 83.8 $\pm$ 3.1 & \textbf{86.9} $\pm$ 2.6 & \textbf{91.2} $\pm$ 1.3 & \textbf{87.0} $\pm$ 3.0\\
walker2d-medium & \textbf{86.0} $\pm$ 0.5 & \textbf{86.1} $\pm$ 0.4 & \textbf{86.2} $\pm$ 0.3 & \textbf{86.2} $\pm$ 0.6 & \textbf{85.5} $\pm$ 0.1 & \textbf{85.9} $\pm$ 0.6\\
ant-medium & \textbf{104.1} $\pm$ 0.6 & \textbf{104.7} $\pm$ 0.5 & \textbf{104.6} $\pm$ 0.3 & \textbf{104.7} $\pm$ 0.7 & \textbf{104.0} $\pm$ 0.5 & \textbf{104.1} $\pm$ 0.6\\
halfcheetah-medium-replay & \textbf{45.7} $\pm$ 0.5 & \textbf{45.7} $\pm$ 0.4 & \textbf{45.8} $\pm$ 0.0 & \textbf{45.7} $\pm$ 0.4 & \textbf{45.6} $\pm$ 0.0 & \textbf{45.8} $\pm$ 0.3\\
hopper-medium-replay & \textbf{99.8} $\pm$ 0.4 & \textbf{100.2} $\pm$ 1.0 & \textbf{100.6} $\pm$ 1.5 & \textbf{100.3} $\pm$ 1.4 & \textbf{98.4} $\pm$ 1.4 & \textbf{99.7} $\pm$ 1.2\\
walker2d-medium-replay & \textbf{89.2} $\pm$ 0.5 & \textbf{89.7} $\pm$ 1.0 & \textbf{88.0} $\pm$ 0.9 & \textbf{88.4} $\pm$ 1.2 & \textbf{88.7} $\pm$ 0.9 & \textbf{87.6} $\pm$ 1.1\\
ant-medium-replay & \textbf{101.8} $\pm$ 0.2 & \textbf{102.6} $\pm$ 1.3 & \textbf{101.2} $\pm$ 0.2 & \textbf{102.0} $\pm$ 1.1 & \textbf{100.3} $\pm$ 1.0 & \textbf{100.6} $\pm$ 1.0\\
		\hline 
Average over datasets & \textbf{91.4} $\pm$ 0.7 & \textbf{91.8} $\pm$ 1.4 & \textbf{89.6} $\pm$ 1.3 & \textbf{89.5} $\pm$ 1.7 & \textbf{89.0} $\pm$ 0.7 & \textbf{88.1} $\pm$ 1.4\\


\end{tabular}}\end{center}\end{table*}

==> tables/new_cql_20seeds_last_four.tex <==
\begin{table*} [htb]\settablefontsize \settablecolsep
\caption{Average last four evaluations for some key experiments with 20 seeds. The number following the pretraining style indicates the total number of pretraining updates. For example, `MDP1m' means pretraining with MDP data for 1M timesteps.}
\label{table:cql-abl-ns-best}
\begin{center}{\begin{tabular}{lllllllllll}

Average Final Four & CQL & IID1m & IID100k & MDP1m & MDP100k & MDP50k & MDP25k & MDP1k & MDP1 \\
		\hline 
halfcheetah-medium-expert & 33.1 $\pm$ 5.1 & \textbf{57.9} $\pm$ 7.4 & 57.4 $\pm$ 6.4 & \textbf{59.3} $\pm$ 6.1 & \textbf{60.9} $\pm$ 7.2 & \textbf{58.9} $\pm$ 8.3 & 53.7 $\pm$ 6.3 & 38.9 $\pm$ 5.7 & 32.7 $\pm$ 4.1\\
hopper-medium-expert & 56.9 $\pm$ 20.3 & \textbf{92.3} $\pm$ 15.7 & 82.8 $\pm$ 17.5 & 81.6 $\pm$ 14.5 & 89.5 $\pm$ 13.2 & \textbf{94.9} $\pm$ 12.2 & 77.0 $\pm$ 20.0 & 76.3 $\pm$ 18.6 & 55.9 $\pm$ 28.2\\
walker2d-medium-expert & \textbf{107.9} $\pm$ 3.8 & \textbf{110.0} $\pm$ 0.4 & \textbf{109.9} $\pm$ 0.4 & \textbf{110.2} $\pm$ 0.3 & \textbf{109.9} $\pm$ 0.3 & \textbf{109.9} $\pm$ 0.5 & \textbf{110.0} $\pm$ 0.2 & \textbf{109.9} $\pm$ 1.0 & \textbf{109.3} $\pm$ 2.2\\
ant-medium-expert & 110.6 $\pm$ 5.4 & \textbf{117.8} $\pm$ 4.9 & \textbf{117.4} $\pm$ 4.4 & \textbf{119.3} $\pm$ 4.5 & \textbf{118.3} $\pm$ 5.4 & \textbf{119.0} $\pm$ 5.2 & \textbf{118.1} $\pm$ 4.1 & 113.3 $\pm$ 4.7 & 110.9 $\pm$ 6.1\\
halfcheetah-medium & \textbf{46.0} $\pm$ 0.2 & \textbf{46.3} $\pm$ 0.2 & \textbf{46.4} $\pm$ 0.2 & \textbf{46.3} $\pm$ 0.2 & \textbf{46.5} $\pm$ 0.2 & \textbf{46.3} $\pm$ 0.2 & \textbf{46.3} $\pm$ 0.2 & \textbf{46.3} $\pm$ 0.2 & \textbf{46.0} $\pm$ 0.2\\
hopper-medium & \textbf{67.4} $\pm$ 4.1 & \textbf{64.6} $\pm$ 2.6 & \textbf{65.6} $\pm$ 3.9 & \textbf{65.3} $\pm$ 3.4 & \textbf{66.3} $\pm$ 4.1 & \textbf{67.3} $\pm$ 2.9 & \textbf{65.9} $\pm$ 2.9 & \textbf{65.4} $\pm$ 3.7 & \textbf{67.4} $\pm$ 3.0\\
walker2d-medium & \textbf{82.2} $\pm$ 1.8 & \textbf{83.2} $\pm$ 0.8 & \textbf{83.3} $\pm$ 0.8 & \textbf{83.4} $\pm$ 1.2 & \textbf{83.4} $\pm$ 1.1 & \textbf{83.3} $\pm$ 0.6 & \textbf{83.0} $\pm$ 0.6 & \textbf{83.2} $\pm$ 1.0 & \textbf{82.5} $\pm$ 1.2\\
ant-medium & 91.2 $\pm$ 4.0 & \textbf{93.5} $\pm$ 4.1 & \textbf{96.0} $\pm$ 2.9 & \textbf{93.2} $\pm$ 4.4 & \textbf{95.5} $\pm$ 3.3 & \textbf{94.7} $\pm$ 3.6 & \textbf{95.7} $\pm$ 2.9 & \textbf{92.4} $\pm$ 4.2 & \textbf{94.5} $\pm$ 4.3\\
halfcheetah-medium-replay & \textbf{44.3} $\pm$ 0.3 & \textbf{44.3} $\pm$ 0.3 & \textbf{44.5} $\pm$ 0.3 & \textbf{44.3} $\pm$ 0.3 & \textbf{44.6} $\pm$ 0.4 & \textbf{44.4} $\pm$ 0.3 & \textbf{44.4} $\pm$ 0.4 & \textbf{44.3} $\pm$ 0.4 & \textbf{44.3} $\pm$ 0.3\\
hopper-medium-replay & \textbf{93.7} $\pm$ 2.3 & \textbf{96.3} $\pm$ 2.4 & \textbf{92.7} $\pm$ 3.0 & \textbf{95.9} $\pm$ 3.3 & \textbf{94.7} $\pm$ 3.2 & \textbf{91.5} $\pm$ 6.9 & \textbf{92.2} $\pm$ 5.4 & \textbf{95.1} $\pm$ 2.7 & \textbf{94.2} $\pm$ 2.2\\
walker2d-medium-replay & 80.0 $\pm$ 4.1 & \textbf{81.7} $\pm$ 2.9 & \textbf{83.2} $\pm$ 2.2 & \textbf{83.2} $\pm$ 1.7 & \textbf{83.9} $\pm$ 2.4 & \textbf{84.4} $\pm$ 1.8 & \textbf{83.5} $\pm$ 2.3 & \textbf{80.6} $\pm$ 3.4 & \textbf{81.0} $\pm$ 1.7\\
ant-medium-replay & 89.0 $\pm$ 3.8 & \textbf{92.9} $\pm$ 4.0 & \textbf{94.2} $\pm$ 5.0 & \textbf{93.8} $\pm$ 3.5 & \textbf{94.3} $\pm$ 3.5 & \textbf{92.4} $\pm$ 4.6 & \textbf{93.9} $\pm$ 4.4 & \textbf{92.2} $\pm$ 4.6 & \textbf{92.4} $\pm$ 4.0\\
		\hline 
Average over datasets & 75.2 $\pm$ 4.6 & \textbf{81.7} $\pm$ 3.8 & \textbf{81.1} $\pm$ 3.9 & \textbf{81.3} $\pm$ 3.6 & \textbf{82.3} $\pm$ 3.7 & \textbf{82.2} $\pm$ 3.9 & \textbf{80.3} $\pm$ 4.1 & 78.2 $\pm$ 4.2 & 75.9 $\pm$ 4.8\\

\end{tabular}}\end{center}\end{table*}


\begin{table*} [htb]\settablefontsize \settablecolsep
\caption{Average last four evaluations for some experiments with 20 seeds and the corresponding old experiments with much fewer seeds. Every two experiments is one pair indicating the old-result column followed by the new-result column (column name ends with 20). The number prefixing the pretraining style is the total number of pretraining timesteps. For example, `1mMDP20' means pretraining with MDP data for 1M timesteps averaged over 20 seeds.}
\label{table:cql-abl-ns-best}
\begin{center}{\begin{tabular}{llllllllllllll}

Average Final Four & CQL & CQL20 & IID & IID20 & 1mMDP & 1mMDP20 \\
		\hline 
halfcheetah-medium-expert & 31.4 $\pm$ 2.7 & 33.1 $\pm$ 5.1 & 53.5 $\pm$ 6.5 & \textbf{57.9} $\pm$ 7.4 & \textbf{60.9} $\pm$ 2.8 & \textbf{59.3} $\pm$ 6.1\\
hopper-medium-expert & 51.2 $\pm$ 25.4 & 56.9 $\pm$ 20.3 & \textbf{92.7} $\pm$ 10.9 & \textbf{92.3} $\pm$ 15.7 & 77.0 $\pm$ 16.9 & 81.6 $\pm$ 14.5\\
walker2d-medium-expert & \textbf{108.1} $\pm$ 0.8 & \textbf{107.9} $\pm$ 3.8 & \textbf{110.2} $\pm$ 0.3 & \textbf{110.0} $\pm$ 0.4 & \textbf{110.0} $\pm$ 0.5 & \textbf{110.2} $\pm$ 0.3\\
ant-medium-expert & 110.2 $\pm$ 2.9 & 110.6 $\pm$ 5.4 & \textbf{116.2} $\pm$ 3.9 & \textbf{117.8} $\pm$ 4.9 & \textbf{115.8} $\pm$ 5.9 & \textbf{119.3} $\pm$ 4.5\\
halfcheetah-medium & \textbf{46.1} $\pm$ 0.1 & \textbf{46.0} $\pm$ 0.2 & \textbf{46.2} $\pm$ 0.2 & \textbf{46.3} $\pm$ 0.2 & \textbf{46.3} $\pm$ 0.1 & \textbf{46.3} $\pm$ 0.2\\
hopper-medium & \textbf{67.1} $\pm$ 4.2 & \textbf{67.4} $\pm$ 4.1 & \textbf{68.3} $\pm$ 1.9 & 64.6 $\pm$ 2.6 & \textbf{68.8} $\pm$ 3.7 & 65.3 $\pm$ 3.4\\
walker2d-medium & \textbf{81.9} $\pm$ 1.8 & \textbf{82.2} $\pm$ 1.8 & \textbf{83.4} $\pm$ 0.7 & \textbf{83.2} $\pm$ 0.8 & \textbf{83.3} $\pm$ 0.5 & \textbf{83.4} $\pm$ 1.2\\
ant-medium & \textbf{93.1} $\pm$ 3.1 & 91.2 $\pm$ 4.0 & \textbf{95.7} $\pm$ 4.8 & \textbf{93.5} $\pm$ 4.1 & \textbf{96.6} $\pm$ 2.1 & \textbf{93.2} $\pm$ 4.4\\
halfcheetah-medium-replay & \textbf{44.4} $\pm$ 0.4 & \textbf{44.3} $\pm$ 0.3 & \textbf{44.2} $\pm$ 0.2 & \textbf{44.3} $\pm$ 0.3 & \textbf{44.3} $\pm$ 0.4 & \textbf{44.3} $\pm$ 0.3\\
hopper-medium-replay & \textbf{94.0} $\pm$ 2.8 & \textbf{93.7} $\pm$ 2.3 & \textbf{95.2} $\pm$ 1.9 & \textbf{96.3} $\pm$ 2.4 & \textbf{96.7} $\pm$ 3.2 & \textbf{95.9} $\pm$ 3.3\\
walker2d-medium-replay & \textbf{79.3} $\pm$ 2.1 & \textbf{80.0} $\pm$ 4.1 & \textbf{82.8} $\pm$ 1.2 & \textbf{81.7} $\pm$ 2.9 & \textbf{82.1} $\pm$ 3.6 & \textbf{83.2} $\pm$ 1.7\\
ant-medium-replay & 88.7 $\pm$ 3.7 & 89.0 $\pm$ 3.8 & \textbf{92.7} $\pm$ 1.3 & \textbf{92.9} $\pm$ 4.0 & \textbf{94.0} $\pm$ 5.0 & \textbf{93.8} $\pm$ 3.5\\
		\hline 
Average over datasets & 74.6 $\pm$ 4.2 & 75.2 $\pm$ 4.6 & \textbf{81.8} $\pm$ 2.8 & \textbf{81.7} $\pm$ 3.8 & \textbf{81.3} $\pm$ 3.7 & \textbf{81.3} $\pm$ 3.6\\

\end{tabular}}\end{center}\end{table*}


\begin{table*} [htb]\settablefontsize \settablecolsep
\caption{Average last four evaluations for some experiments with 20 seeds and the corresponding old experiments with much fewer seeds. Every two experiments is one pair indicating the old-result column followed by the new-result column (column name ends with 20). The number prefixing the pretraining style is the total number of pretraining timesteps. For example, `1mMDP20' means pretraining with MDP data for 1M timesteps averaged over 20 seeds.}
\label{table:cql-abl-ns-best}
\begin{center}{\begin{tabular}{llllllllllllll}

Average Final Four & 50kMDP & 50kMDP20 & 1kMDP & 1kMDP20 & 1MDP & 1MDP20 \\
		\hline 
halfcheetah-medium-expert & \textbf{66.2} $\pm$ 0.0 & 58.9 $\pm$ 8.3 & 40.5 $\pm$ 5.6 & 38.9 $\pm$ 5.7 & 38.8 $\pm$ 7.5 & 32.7 $\pm$ 4.1\\
hopper-medium-expert & 79.3 $\pm$ 14.5 & \textbf{94.9} $\pm$ 12.2 & 73.6 $\pm$ 11.7 & 76.3 $\pm$ 18.6 & 84.9 $\pm$ 5.9 & 55.9 $\pm$ 28.2\\
walker2d-medium-expert & \textbf{110.3} $\pm$ 0.1 & \textbf{109.9} $\pm$ 0.5 & \textbf{109.5} $\pm$ 0.3 & \textbf{109.9} $\pm$ 1.0 & \textbf{107.7} $\pm$ 2.3 & \textbf{109.3} $\pm$ 2.2\\
ant-medium-expert & \textbf{119.7} $\pm$ 2.4 & \textbf{119.0} $\pm$ 5.2 & \textbf{115.3} $\pm$ 7.3 & 113.3 $\pm$ 4.7 & 110.0 $\pm$ 3.6 & 110.9 $\pm$ 6.1\\
halfcheetah-medium & \textbf{46.4} $\pm$ 0.1 & \textbf{46.3} $\pm$ 0.2 & \textbf{46.3} $\pm$ 0.2 & \textbf{46.3} $\pm$ 0.2 & \textbf{46.1} $\pm$ 0.0 & \textbf{46.0} $\pm$ 0.2\\
hopper-medium & 63.8 $\pm$ 1.6 & \textbf{67.3} $\pm$ 2.9 & 62.2 $\pm$ 6.8 & \textbf{65.4} $\pm$ 3.7 & \textbf{66.5} $\pm$ 2.2 & \textbf{67.4} $\pm$ 3.0\\
walker2d-medium & \textbf{81.6} $\pm$ 1.1 & \textbf{83.3} $\pm$ 0.6 & \textbf{82.7} $\pm$ 1.3 & \textbf{83.2} $\pm$ 1.0 & \textbf{83.3} $\pm$ 0.9 & \textbf{82.5} $\pm$ 1.2\\
ant-medium & \textbf{94.3} $\pm$ 1.7 & \textbf{94.7} $\pm$ 3.6 & \textbf{98.9} $\pm$ 3.0 & 92.4 $\pm$ 4.2 & 89.4 $\pm$ 3.7 & \textbf{94.5} $\pm$ 4.3\\
halfcheetah-medium-replay & \textbf{44.2} $\pm$ 0.1 & \textbf{44.4} $\pm$ 0.3 & \textbf{44.3} $\pm$ 0.1 & \textbf{44.3} $\pm$ 0.4 & \textbf{44.2} $\pm$ 0.2 & \textbf{44.3} $\pm$ 0.3\\
hopper-medium-replay & \textbf{95.3} $\pm$ 1.9 & \textbf{91.5} $\pm$ 6.9 & \textbf{94.9} $\pm$ 2.1 & \textbf{95.1} $\pm$ 2.7 & \textbf{92.3} $\pm$ 2.4 & \textbf{94.2} $\pm$ 2.2\\
walker2d-medium-replay & \textbf{83.5} $\pm$ 1.1 & \textbf{84.4} $\pm$ 1.8 & \textbf{81.9} $\pm$ 2.0 & \textbf{80.6} $\pm$ 3.4 & \textbf{82.9} $\pm$ 3.7 & \textbf{81.0} $\pm$ 1.7\\
ant-medium-replay & 89.9 $\pm$ 6.1 & \textbf{92.4} $\pm$ 4.6 & \textbf{92.9} $\pm$ 4.5 & \textbf{92.2} $\pm$ 4.6 & \textbf{94.9} $\pm$ 3.1 & \textbf{92.4} $\pm$ 4.0\\
		\hline 
Average over datasets & \textbf{81.2} $\pm$ 2.5 & \textbf{82.2} $\pm$ 3.9 & \textbf{78.6} $\pm$ 3.8 & \textbf{78.2} $\pm$ 4.2 & \textbf{78.4} $\pm$ 3.0 & 75.9 $\pm$ 4.8\\


\end{tabular}}\end{center}\end{table*}

==> tables/new_cql_main_table_best.tex <==
\begin{table*} [htb]\settablefontsize \settablecolsep
\caption{Best test score for CQL and CQL + Synthetic pretraining. For CQL + Synthetic variant, the MDP dataset by default has a state space of size 100, an action space of size 100, and a temperature of 1 for both the policy distribution and the transition probability distribution. }
\label{table:cql-main-best}
\begin{center}{\begin{tabular}{llllllll}

Best Score & CQL & CQL+MDP & CQL+IID \\
		\hline 
halfcheetah-medium-expert & 44.6 $\pm$ 6.4 & \textbf{84.7} $\pm$ 4.2 & 79.1 $\pm$ 5.4\\
hopper-medium-expert & \textbf{106.7} $\pm$ 6.6 & \textbf{111.2} $\pm$ 0.3 & \textbf{111.5} $\pm$ 0.5\\
walker2d-medium-expert & \textbf{112.1} $\pm$ 0.5 & \textbf{112.4} $\pm$ 0.6 & \textbf{114.0} $\pm$ 1.5\\
ant-medium-expert & \textbf{128.7} $\pm$ 0.9 & \textbf{130.6} $\pm$ 0.7 & \textbf{129.7} $\pm$ 0.8\\
halfcheetah-medium & \textbf{46.9} $\pm$ 0.1 & \textbf{47.3} $\pm$ 0.1 & \textbf{47.1} $\pm$ 0.2\\
hopper-medium & \textbf{86.5} $\pm$ 4.7 & \textbf{85.4} $\pm$ 1.1 & \textbf{87.8} $\pm$ 3.4\\
walker2d-medium & \textbf{85.6} $\pm$ 0.4 & \textbf{86.0} $\pm$ 0.3 & \textbf{86.2} $\pm$ 0.3\\
ant-medium & \textbf{103.5} $\pm$ 0.7 & \textbf{104.9} $\pm$ 0.6 & \textbf{104.4} $\pm$ 0.9\\
halfcheetah-medium-replay & \textbf{45.7} $\pm$ 0.2 & \textbf{45.7} $\pm$ 0.4 & \textbf{45.4} $\pm$ 0.2\\
hopper-medium-replay & \textbf{100.2} $\pm$ 1.4 & \textbf{101.0} $\pm$ 1.2 & \textbf{100.5} $\pm$ 0.6\\
walker2d-medium-replay & \textbf{88.3} $\pm$ 1.6 & \textbf{89.5} $\pm$ 1.1 & \textbf{89.3} $\pm$ 1.3\\
ant-medium-replay & \textbf{99.5} $\pm$ 1.5 & \textbf{102.5} $\pm$ 0.7 & \textbf{101.8} $\pm$ 0.6\\
		\hline 
Average over datasets & \textbf{87.3} $\pm$ 2.1 & \textbf{91.8} $\pm$ 0.9 & \textbf{91.4} $\pm$ 1.3\\


\end{tabular}}\end{center}\end{table*}

==> tables/new_cql_main_table_last_four.tex <==
\begin{table*} [htb]\settablefontsize \settablecolsep
\caption{Final performance for CQL with synthetic pre+training. The MDP pre-training dataset by default has state and action sizes of 100 and a temperature of 1 for both the policy distribution and the transition probability distribution.}
\label{table:cql-main-last-four}

\begin{center}{\begin{tabular}{llllllll}

Average Final Four & CQL & CQL+MDP & CQL+IID \\
		\hline 
halfcheetah-medium-expert & 31.4 $\pm$ 2.7 & \textbf{60.9} $\pm$ 2.8 & 53.5 $\pm$ 6.5\\
hopper-medium-expert & 51.2 $\pm$ 25.4 & 77.0 $\pm$ 16.9 & \textbf{92.7} $\pm$ 10.9\\
walker2d-medium-expert & \textbf{108.1} $\pm$ 0.8 & \textbf{110.0} $\pm$ 0.5 & \textbf{110.2} $\pm$ 0.3\\
ant-medium-expert & 110.2 $\pm$ 2.9 & \textbf{115.8} $\pm$ 5.9 & \textbf{116.2} $\pm$ 3.9\\
halfcheetah-medium & \textbf{46.1} $\pm$ 0.1 & \textbf{46.3} $\pm$ 0.1 & \textbf{46.2} $\pm$ 0.2\\
hopper-medium & \textbf{67.1} $\pm$ 4.2 & \textbf{68.8} $\pm$ 3.7 & \textbf{68.3} $\pm$ 1.9\\
walker2d-medium & \textbf{81.9} $\pm$ 1.8 & \textbf{83.3} $\pm$ 0.5 & \textbf{83.4} $\pm$ 0.7\\
ant-medium & \textbf{93.1} $\pm$ 3.1 & \textbf{96.6} $\pm$ 2.1 & \textbf{95.7} $\pm$ 4.8\\
halfcheetah-medium-replay & \textbf{44.4} $\pm$ 0.4 & \textbf{44.3} $\pm$ 0.4 & \textbf{44.2} $\pm$ 0.2\\
hopper-medium-replay & \textbf{94.0} $\pm$ 2.8 & \textbf{96.7} $\pm$ 3.2 & \textbf{95.2} $\pm$ 1.9\\
walker2d-medium-replay & \textbf{79.3} $\pm$ 2.1 & \textbf{82.1} $\pm$ 3.6 & \textbf{82.8} $\pm$ 1.2\\
ant-medium-replay & 88.7 $\pm$ 3.7 & \textbf{94.0} $\pm$ 5.0 & \textbf{92.7} $\pm$ 1.3\\
		\hline 
Average over datasets & 74.6 $\pm$ 4.2 & \textbf{81.3} $\pm$ 3.7 & \textbf{81.8} $\pm$ 2.8\\


\end{tabular}}\end{center}\end{table*}
